OptiRica: Towards an Efficient Optimizing Horn Solver

This paper describes an ongoing effort to develop an optimizing version of the Eldarica Horn solver. The work starts from the observation that many kinds of optimization problems, and in particular the MaxSAT/SMT problem, can be seen as search problems on lattices. The paper presents a Scala library providing a domain-specific language (DSL) to uniformly model optimization problems of this kind, by defining, manipulating, and systematically exploring lattices with associated objective functions. The framework can be instantiated to obtain an optimizing Horn solver. As an illustration, the application of an optimizing solver for repairing software-defined networks is described.

==> eptcsdata.tex <==
\providecommand{\firstpage}{35}
\providecommand{\publicationstatus}{G.W. Hamilton, T. Kahsai, M. Proietti (Eds.):\\
Joint International Workshops on \\
Horn Clauses for Verification and Synthesis (HCVS 2022)\\
Verification and Program Transformation (VPT 2022)\\
EPTCS 373, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.373.4}{10.4204/EPTCS.373.4}}

